Cofibrance and Completion

For a cofibrantly generated Quillen model category, we show that the cofibrant replacement functor constructed using the small object argument admits a cotriple structure. If all acyclic cofibrations are monomorphisms, the fibrant replacement functor constructed using the small object argument admits a triple structure. For a triple in the base category, the associated cosimplicial resolution is not necessarily homotopy invariant. However using a mix of the triple with the cofibrant replacement cotriple we construct a 'homotopically correct' version of the cosimplicial resolution of the triple. This allows us to construct a Bousfield-Kan completion functor with respect to a triple, and for pointed cofibrantly-generated model categories a Bousfield-Kan spectral sequence that computes the relative homotopy groups of the Bousfield-Kan completion of an object. This is the text of my PhD thesis, worked under the supervision of Prof. Haynes Miller, submitted on Feb. 1999 at MIT.

==> garbage.tex <==
\bigskip
\bigskip

\subsection{A second description of $X. \tens K.$ and ${(Y \tdot)}^{K.}$}
\label{subsecBC4}
There is a second, more abstract way to describe the functors $X. \tens K.$ and $(Y \tdot)^{K.}$. 
Fix the simplicial set $K.$
There is a map of simplicial sets $K. \ra *$ to the point.
This yields a functor 
\begin{center}
$u_K$ : $\Delta K. \lra \Delta * = \Delta$
\end{center}
Consider the following pairs of adjoint functors

\bigskip

\begin{center}
$\colim^{(u^{op}_K)^*} : {\cat C}^{(\Delta K.)^{op}} \xymatrix{ \ar@<.5ex>[r] & \ar@<.5ex>[l] } {\cat C}^{\Delta^{op}} : (u^{op}_K)^*$

\bigskip

$u^*_K : {\cat C}^\Delta \xymatrix{ \ar@<.5ex>[r] & \ar@<.5ex>[l] } {\cat C}^{\Delta K.} : \lim^{u^*_K}$
\bigskip
\end{center}
where $\colim^{(u^{op}_K)^*}$ denotes the left Kan extension along $u^{op}_K$ and $\lim^{u^*_K}$ denotes the right Kan extension along $u_K$.
Using the standard description of Kan extensions (see for example \cite{Dwyer-Kan-Hirschhorn}, 43.2),

\begin{center}
 $(\colim^{(u^{op}_K)^*} A)_n$ $=$ $\colim^{(u^{op}_K \downarrow \underline{n})} A$ 
\end{center}
Here $(u^{op}_K \downarrow \underline{n})$ denotes the over category of the functor $u^{op}_K$ : $(\Delta K.)^{op} \lra \Delta^{op}$ with respect to object $\underline{n}$ of $\Delta^{op}$. 
$A$ is a ${(\Delta K.)^{op}}$- diagram in ${\cat C}$.
Similarly, 

\begin{center}
 $(\lim^{u^*_K} B)^n$ $=$ $\lim^{(\underline{n} \downarrow u_K)} B$ 
\end{center}
$(\underline{n} \downarrow u_K)$ denotes the under category of $u_K$ : $\Delta K. \lra \Delta$ at object $\underline{n}$ of $\Delta$.
$B$ is a $\Delta K.$- diagram in ${\cat C}$.

\bigskip

\begin{prop}
\label{propBC5}
There are natural isomorphisms of functors 
\begin{center}
$X. \tens K.$ $\cong$ $\colim^{(u^{op}_K)^*} (u^{op}_K)^* X.$

$(Y \tdot)^{K.}$ $\cong$ $\lim^{u^*_K} (u^*_K Y \tdot)$
\end{center}
\end{prop}

\begin{proof}
We prove existence of the first canonical isomorphism - the second one follows by duality.

Fix $K.$ , and for ease of notation denote $v = u^{op}_K$ : $(\Delta K.)^{op} \lra \Delta^{op}$.

We want to compute $\colim^{v^*} (v^* X.)$ -we will show that 
\begin{equation}
\label{eqnBC4}
(\mathrm{colim}^{v^*} (v^* X.))_n = \sqcup_{K_n} X_n
\end{equation}
We will skip the proof that this isomorphism is compatible with respect to face and degeneracy maps, and also the proof of naturality. 

\bigskip

Observe that 
\begin{center}
$Ob(\Delta K.)^{op}$ $\cong$ $K_0 \cup K_1 \cup$ ... $K_n \cup$ ... 
\end{center}
The equation (\ref{eqnBC4}) will be a consequence of the canonical isomorphism
\begin{equation}
\label{eqnBC6}
(\mathrm{colim}^{v^*} A)_n = \sqcup_{x \in K_n} A_x
\end{equation}
where $A \in Ob{\cat C}^{(\Delta K.)^{op}}$.

We have that 
\begin{center}
$(\colim^{v^*} A)_n = \colim^{(v \downarrow \underline{n})} A$
\end{center}

The category $(v \downarrow \underline{n}) = (\underline{n} \downarrow v^{op})^{op}$ has, as objects, maps in $\Delta$ of the form
\begin{center}
$\underline{n} \xymatrix{\ar[r]^a &} v^{op}(x)$ 
\end{center}
where $x \in Ob(\Delta K.)$ is a simplicial set map
\begin{center}
$\Delta[k] \xymatrix{\ar[r]^x &} K.$ 
\end{center}
Therefore, we actually have $v^{op}(x) = \underline{k}$.
Denote this object of $(\underline{n} \downarrow v^{op})$ by $(a,x)$.

The category $(\underline{n} \downarrow v^{op})^{op}$ has, as maps from $(a,x)$ to $(b,y)$, commutative diagrams of the form
\begin{center}
$\xymatrix{
	\Delta[k] \ar[r]^x &
	K. \\
	& \Delta[l] \ar[u]_y \ar[ul]^f 
}$
\end{center}
with the property that the diagram in $\Delta$ shown below is commutative:
\begin{center}
$\xymatrix{
	& {\underline{k}} \\
	{\underline{n}} \ar[ur]^a \ar[r]_b &
	{\underline{l}} \ar[u]_f
}$
\end{center}

One observes that the category $(\underline{n} \downarrow v^{op})^{op}$ has, as a terminal subcategory, the discrete subcategory denoted ${\cat D}_n$, with objects $(a,x)$, with 
\begin{center}
$\Delta[n] \xymatrix{\ar[r]^x &} K.$ \phantom{po} and \phantom{po} 
$\underline{n} \xymatrix{\ar[r]^a_{id} &} v^{op}(x) = \underline{n}$
\end{center}

\bigskip

Since ${\cat D}_n$ is a terminal subcategory of $(\underline{n} \downarrow v^{op})^{op} = (v \downarrow \underline{n})$,
\begin{center}
$\colim^{(v \downarrow \underline{n})} A = \colim^{{\cat D}_n} A = \sqcup_{x \in K_n} A_x$
\end{center}
\end{proof}

\newpage

\begin{lemma}
\label{lemmaBC1}
Fix $K.$ a simplicial set.
Then both of the adjoint functors 
\begin{center}
$\colim^{(u^{op}_K)^*} : {\cat M}^{(\Delta K.)^{op}} \xymatrix{ \ar@<.5ex>[r] & \ar@<.5ex>[l] } {\cat M}^{\Delta^{op}} : (u^{op}_K)^*$
\end{center}
carry weak equivalences to weak equivalences.
\end{lemma} 

\begin{proof}
If $X. \ra Y.$ is a weak equivalence in ${\cat M}^{\Delta^{op}}$, then since $X_n \xymatrix{\ar[r]^\sim &} Y_n$ we get that 
\begin{center}
$(u^{op}_K)^*X. \xymatrix{\ar[r]^\sim &} (u^{op}_K)^*Y.$ 
\end{center}
is a weak equivalence in ${\cat M}^{(\Delta K.)^{op}}$

\bigskip

Let $A \ra B$ be a weak equivalence in ${\cat M}^{(\Delta K.)^{op}}$.

This means that for any object $x \in Ob(\Delta K.)^{op}$ = $K_0 \cup K_1 \cup$ ... $K_n \cup$ ... we have
\begin{center}
$A_x \xymatrix{\ar[r]^\sim &} B_x$
\end{center}
and by (\ref{eqnBC6})
\begin{center}
$\colim^{(u^{op}_K)^*}A \xymatrix{\ar[r]^\sim &} \colim^{(u^{op}_K)^*}B$ 
\end{center}
is a weak equivalence
\end{proof}
\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reduction to the Diagonal}
\label{secRedDiag}

\bigskip
\bigskip

Let ${\cat M}$ be a model category.

\begin{lemma}
\label{lemmaBK1}
If $X..$ is a bi-simplicial object in ${\cat M}$ (  $X.. \in Ob({\cat M}^{\Delta^{op} \times \Delta^{op}})$), then the natural map below is an equivalence
\begin{center}
${\mathbf L}\colim^{\Delta^{op}} diag(X..) \ra {\mathbf L}\colim^{\Delta^{op} \times \Delta^{op}} X..$ 
\end{center}

Dually, if $Y \tdotdot \in Ob({\cat M}^{\Delta \times \Delta})$ then
\begin{center}
${\mathbf R}\lim^{\Delta \times \Delta} Y \tdotdot \ra {\mathbf R}\lim^\Delta diag(Y \tdotdot)$
\end{center}
is an equivalence.
\end{lemma}

\begin{proof}
We also denote by $diag$ the diagonal functor $\Delta \ra \Delta \times \Delta$.

Based on Dwyer, Hirschhorn and Kan's (\cite{Dwyer-Kan-Hirschhorn}) Cofinality Theorem 62.3, all we have to show is that the functor $diag$: $\Delta \ra \Delta \times \Delta$ is initial.

Let $(\underline{k_1},\underline{k_2}) \in Ob(\Delta \times \Delta)$.
We have to show that the nerve of the category $(diag \downarrow (\underline{k_1},\underline{k_2}))$ is contractible.
We use the convention that the nerve of a category ${\cat C}$ is denoted also ${\cat C}$.

\bigskip

If $K$ is a simplicial set, $\Delta K$  (the ``barycentric subdivision'') denotes the category with
\begin{list}{-}{}
 \item $Ob \Delta K$ = simplicial set maps of the form $\Delta[n] \ra K$
 \item $Hom_{\Delta K}(a, b)$ = commutative diagrams
\begin{center}
$\xymatrix{
	\Delta[n] \ar[r]^a \ar[dr] &
	K \\
	& \Delta[m] \ar[u]_b
}$
\end{center}
\end{list}

A known result is that $\Delta K$ has the same homotopy type as $K$.

\bigskip

It is easy to see that
\begin{equation}
\label{eqnRedd1}
Hom_{sSets}(\Delta[n], \Delta[k]) = Hom_\Delta(\underline{n}, \underline{k})
\end{equation}
As a consequence, we have an isomorphism of categories
\begin{equation}
\label{eqnBC3}
(diag \downarrow (\underline{k_1},\underline{k_2})) = \Delta(\Delta[k_1] \times \Delta[k_2])
\end{equation}
To prove this, observe that an object of $(diag \downarrow (\underline{k_1},\underline{k_2}))$ is a pair of maps in $\Delta$
\begin{center}
$\xymatrix{
	{\underline{n}} \ar[r]^{a_1} & 
	{\underline{k_1}}
}$

$\xymatrix{
	{\underline{n}} \ar[r]^{a_2} & {\underline{k_2}}
}$
\end{center}
and can be identified using (\ref{eqnRedd1}) with a simplicial set map
\begin{center}
$\xymatrix{
	\Delta[n] \ar[rr]^(.4){a_1 \times a_2} & &
	\Delta[k_1] \times \Delta[k_2]
}$
\end{center}

\bigskip

It follows from (\ref{eqnBC3}) that $(diag \downarrow (\underline{k_1},\underline{k_2}))$ has the homotopy type of $\Delta[k_1] \times \Delta[k_2]$, therefore it is contractible. 
This ends the proof.
\end{proof}

\bigskip
\bigskip
\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Consider a pair of small categories (${\cat C}$, ${\cat W}$) (this means, ${\cat W}$ a subcategory of ${\cat C}$) with $Ob{\cat C}=Ob{\cat W}$.
When ${\cat C} = {\cat M}$ is a model category, we always take ${\cat W}$ to be the subcategory of weak equivalences.

We will construct the function complex ${\bf Hom}(X,Y)$ between any two objects $X$, $Y$ of ${\cat C}$.

To that end, we first outline Dwyer and Kan's construction of simplicial localization of categories (\cite{Dwyer-Kan1}, \cite{Dwyer-Kan2}):

\bigskip

We fix a set ${\cat O}$, and form a category $s{\cat O}$-$Cat$, as below:
\begin{list}{-}{}
 \item its objects are categories ${\cat C}$ enriched over simplicial sets, having ${\cat O}$ as objects: $Ob({\cat C})$ = ${\cat O}$.
Since ${\cat O}$ is a set, such categories ${\cat C}$ are small. 
 \item its maps are simplicial functors $F : {\cat C}_1 \ra {\cat C}_2$ constant on objects: $F(X)$ = $X$, for all $X \, \eps \, {\cat O}$.
\end{list}

We define weak equivalences and fibrations in $s{\cat O}$-$Cat$: a map $F : {\cat C}_1 \ra {\cat C}_2$ is a weak equivalence (resp. fibration) if $F : Hom_{{\cat C}_1}(X,Y) \ra Hom_{{\cat C}_2}(X,Y)$ is a weak equivalence (resp. fibration) of simplicial sets, for all $X$, $Y \, \eps \, {\cat O}$.

With this structure, $s{\cat O}$-$Cat$ becomes a cofibrantly generated model category (\cite{Dwyer-Kan1}).
 
\bigskip
	
Denote $s{\cat O}$-$Cat'$ the category of maps of $s{\cat O}$-$Cat$.
Define weak equivalences in $s{\cat O}$-$Cat'$ as pointwise.

\bigskip

We have a simplicial localization functor ${\cat F}$: $s{\cat O}$-$Cat' \ra s{\cat O}$-$Cat$, given by
\begin{center}
${\cat F}$: (${\cat C}_1 \ra {\cat C}_2$) $\mapsto$ ${\cat C}_2[({{\cat C}_1}^{-1})]$
\end{center}

\bigskip

Dwyer and Kan (\cite{Dwyer-Kan1}) prove that the simplicial localization functor ${\cat F}$ admits a left derived ${\bf L}{\cat F}$: ${\bf ho}(s{\cat O}$-$Cat') \ra {\bf ho}(s{\cat O}$-$Cat)$.
They show this by constructing a convenient model category structure on $s{\cat O}$-$Cat'$, such that ${\cat F}$ carries equivalences between cofibrant objects in $s{\cat O}$-$Cat'$ to equivalences in $s{\cat O}$-$Cat$.

${\bf L}{\cat F}$ is called the simplicial localization functor.

\bigskip
\bigskip

Let (${\cat C}$, ${\cat W}$) be a pair of small categories with $Ob{\cat C}$ = $Ob{\cat W}$ = ${\cat O}$.
 
Of course, regarding the hom-sets of ${\cat C}$ as constant simplicial sets, we have that  ${\cat W} \ra {\cat C}$ is an object of $s{\cat O}$-$Cat'$.

Construct the simplicial localization ${\bf L}{\cat F}({\cat W} \ra {\cat C})$, and define the function complex ${\bf Hom}(X,Y)$ as $Hom_{{\bf L}{\cat F}({\cat W} \ra {\cat C})}(X,Y)$.

Observe that in fact ${\bf Hom}($-$,$-$)$ is a homotopy type of diagrams of simplicial sets in $sSets^{{\cat C}^{op}\times{\cat C}}$, that is, an object of ${\bf ho}(sSets^{{\cat C}^{op}\times{\cat C}})$.

\bigskip

If ${\cat C} = {\cat M}$ is a model category, $Ob{\cat M}=Ob{\cat W}$ is a class and of course there's no problem in performing these constructions in the category $Classes$ as opposed to the category $Sets$.

We have:
\begin{thm}
\label{thmC1}
For an arbitrary model category ${\cat M}$, fix a framing. 
Then there exist natural isomorphisms in ${\bf ho}(sClasses^{{\cat M}^{op}\times{\cat M}})$
\begin{center}
${\bf Hom}(X,Y) $ $\cong$ $ Hom_{\cat M}({\bf X \tdot}, Y') $ $\cong$ $
Hom_{\cat M}(X', {\bf Y .}) $ $\cong$ $ {\bf diag} Hom_{\cat M}({\bf X \tdot}, {\bf Y .})$
\end{center}

Here $X'$ is a canonical cofibrant replacement of $X$, ${\bf X \tdot}$ the cosimplicial frame of $X'$, $Y'$ is a canonical fibrant replacement of $Y$ and ${\bf Y .}$ the simplicial frame of $Y'$.
${\bf diag}$ denotes the diagonal of a bisimplicial set.
\end{thm}

\begin{proof}
See \cite{Dwyer-Kan3}, 4.4. and its proof.
\end{proof}

As a consequence, for a not necessarily small model category ${\cat M}$, ${\bf Hom}(X,Y)$ is {\bf homotopically small} for $X$, $Y \, \eps \, Ob({\cat M})$, that is, it has the homotopy type of a simplicial {\it set}.

Even more than that is true.
If ${\cat M}$ is a model category, by Theorem \ref{thmC1}, the function complex ${\bf Hom}($-$,$-$) \in Ob({\bf ho}(sClasses^{{\cat M}^{op}\times{\cat M}}))$ descends, obviously in a unique way, to an object in ${\bf ho}(sSets^{{\cat M}^{op}\times{\cat M}})$.

From now on, we will allways consider the function complex ${\bf Hom}($-$,$-$)$ as an object of ${\bf ho}(sSets^{{\cat M}^{op}\times{\cat M}})$.

\bigskip





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Effect of Homotopic Maps on Homotopy Limits}
\label{secHomCosMaps2}

\bigskip
\bigskip

In preparation for this section, we prove four lemmas:

\begin{lemma}
\label{lemmaHCM1}
Let ${\cat C}$ be a category as in the previous section, let $A \in Ob{\cat C}$ and $K.$ be a simplicial set.
Regard $A$ as a constant cosimplicial object in ${\cat C}$.
Then there is a natural isomorphism of objects in ${\cat C}^\Delta$ 
\begin{center}
$cosk^n(A^{K.})$ $\cong$ $A^{sk_n K.}$
\end{center}
\end{lemma}

\begin{proof}
Taking into account Chap. \ref{chapHSS}, Proposition \ref{propSkCosk1} that gives a description of $cosk^n$ in terms of matching spaces $M_n(-)$, this lemma is an easy consequence of the natural isomorphism below
\begin{center}
$M_n(A^{K.})$ $\cong$ $\times_{(sk_{n-1}K)_n} A$
\end{center}
This isomorphism in turn follows from the definition of a matching space ({\it nn.} not included here, but see either \cite{Dwyer-Kan-Hirschhorn}, \cite{Hirschhorn} or \cite{Hovey}) and the following rather trivial result:
If $D_i$ is a ${\cat D}$- diagram of simplicial sets and $A \in Ob{\cat C}$, there is a canonical isomorphism in ${\cat C}$
\begin{center}
$\times_{\colim^{\cat D}D_i} A$ $\cong$ $\lim^{\cat D} (\times_{D_i} A)$
\end{center}
\end{proof}

\bigskip

\begin{lemma}
\label{lemmaHCM4}
Let ${\cat M}$ be a model category, let $A \in Ob{\cat M}$ be fibrant and $K.$ be a simplicial set.
Then $A^{K.}$ is Reedy fibrant in ${\cat M}^\Delta$
\end{lemma}

\begin{proof}
This is yet another consequence of the natural isomorphism
\begin{center}
$M_n(A^{K.})$ $\cong$ $\times_{(sk_{n-1}K)_n} A$
\end{center}
\end{proof}
\bigskip

\begin{lemma}
\label{lemmaHCM2}
Let $A.$ be a simplicial set, and regard it as a constant object in $sSets^\Delta$. 
Let $K.$ be a simplicial set.
Then there is a natural isomorphism
\begin{center}
$tot(A. \!^{K.})$ $\cong$ $hom(K. \, , A.)$
\end{center}
where $hom(K. , A.)$ denotes the simplicial hom-set given by 
\begin{center}
$hom(K. \, ,A.)_n$ = $Hom_{sSets}(K. \times \Delta[n], A.)$
\end{center}
\end{lemma}

\begin{proof}
We will use the adjunction (\ref{eqnAdj2})
\begin{center}
$(- \times \Delta \tdot)$ : $sSets \xymatrix{ \ar@<.5ex>[r] & \ar@<.5ex>[l] } sSets^\Delta$  : $tot$
\end{center}

It suffices to show that
\begin{center}
$Hom_{sSets}(B. \,, tot(A. \!^{K.}))$ $\cong$ $Hom_{sSets}(B. \times K. \,, A.)$ 
\end{center}

We have
\begin{center}
$Hom_{sSets}(B. \,, tot(A. \!^{K.}))$ $\cong$ 
$Hom_{sSets^{\Delta^{op}}}(B. \times \Delta \tdot, A.\!^{K.})$ 
\end{center}

This is the same as the set of maps
\begin{center}
$\sqcup_{K_p} (B_p \times \Delta[q]_p) \lra A_p$
\end{center}
that are compatible with maps $d_i$, $s_i$ in the variable $p$, and compatible with maps $d^i$, $s^i$ in the variable $q$.

But in any category ${\cat C}$, $Hom_{{\cat C}^\Delta} (X \tdot, cY)$ = $Hom_{\cat C} (X^0 , Y)$.

Therefore our set of maps is the same as the set of maps of simplicial sets 
\begin{center}
$\sqcup_{K_p} B_p \lra A_p$
\end{center}
which is the same as $Hom_{sSets}(B. \times K. \, , A.)$ .
\end{proof}

\bigskip

\begin{lemma}
\label{lemmaHCM3}
Let $A$ be a simplicial set, and regard it as a constant object in $sSets^\Delta$. 
Let $K.$ be a simplicial set.
Then there is a natural isomorphism
\begin{center}
$tot^n(A. \!^{K.})$ $\cong$ $hom(sk_n K. \, , A.)$
\end{center}
\end{lemma}

\begin{proof}
We have by Chap. \ref{chapHSS}, Prop. \ref{propTotCotot1} and by Lemmas \ref{lemmaHCM1}, \ref{lemmaHCM2}  that
\begin{center}
$tot^n(A. \!^{K.})$ $\cong$ $tot(cosk^n (A. \!^{K.}))$ $\cong$ $tot(A. \!^{sk_n K.})$ $\cong$ $hom(sk_n(K.) \, , A.)$
\end{center}


\end{proof}

\bigskip
\bigskip

We are now ready to for the main results of this section.
Let ${\cat M}$ be a model category. 

\begin{thm}
\label{thmHomot1}
Suppose we have in ${\cat M}^{\Delta^{op}}$ two homotopic maps 
\begin{center}
$f$ $\simeq$ $g$: $X. \lra Y.$ 
\end{center}
Then ${\mathbf L}\colim^{\Delta^{op}} f$ = ${\mathbf L}\colim^{\Delta^{op}} g$
\end{thm}

Dually
\begin{thm}
\label{thmHomot2}
Suppose we have in ${\cat M}^\Delta$ two homotopic maps 
\begin{center}
$f$ $\simeq$ $g$ : $X \tdot \lra Y \tdot$ 
\end{center}
Then ${\mathbf R}\lim^\Delta f$ = ${\mathbf R}\lim^\Delta g$
\end{thm}

\bigskip

In the terminology of Chap. \ref{chapHSS}, Subsection \ref{subsecTotCotot}, these theorems are saying that if $f$ $\simeq$ $g$ : $X. \lra Y.$ then ${\bf cotot}f$ = ${\bf cotot}g$ and dually, if $f$ $\simeq$ $g$ : $X \tdot \lra Y \tdot$ then ${\bf tot}f$ = ${\bf tot}g$.


\begin{proof}
It is enough to prove Theorem \ref{thmHomot2}, for the case ${\cat M}$ = $sSets$.

If $f$ $\simeq$ $g$ : $X. \lra Y.$ are homotopic, then for $Z \in {\cat M}$ the two maps below are naturally homotopic

\begin{center}
${\bf Hom}(f, Z)$ $\simeq$ ${\bf Hom}(g, Z)$ 
\end{center}

By our assumption that Theorem \ref{thmHomot2} is true for ${\cat M}$ = $sSets$ it follows that 

\begin{center}
${\bf tot} \; {\bf Hom}(f, Z)$ = ${\bf tot} \; {\bf Hom}(g, Z)$ 
\end{center}

thererefore 

\begin{center}
${\bf Hom}({\bf cotot}f, Z)$ = ${\bf Hom}({\bf cotot}g, Z)$

\bigskip

${\bf cotot}f$ = ${\bf cotot}g$.
\end{center}

A similar trick works for $f$ $\simeq$ $g$ : $X \tdot \lra Y \tdot$

\bigskip

So let's prove Theorem \ref{thmHomot2} for ${\cat M}$ = $sSets$. 


Denote $H$ a homotopy $f$ $\simeq$ $g$ : $X \tdot \lra Y \tdot$

Because there is a commutative diagram
\begin{center}
$\xymatrix{ & Y \tdot \cong (Y \tdot)^{\Delta[0]} \\ 
	X \tdot \ar[r]^H \ar[ur]^f \ar[dr]_g &
	(Y \tdot)^{\Delta[1]} \ar[u]_{Y^{d^0}} \ar[d]^{Y^{d^1}}  \\
	& Y \tdot \cong (Y \tdot)^{\Delta[0]} 
}$  
\end{center}
one sees that all we have to show is that 
\begin{center}
${\bf R}\lim^\Delta ((Y \tdot) ^{d^0})$ = ${\bf R}\lim^\Delta ((Y \tdot) ^{d^1})$
\end{center}

\bigskip

Both $(Y \tdot)^{d^0}$, $(Y \tdot)^{d^1}$ are sections of 
\begin{equation}
\label{eqnBK8}
\xymatrix{
	(Y \tdot)^{\Delta[0]} \ar[rr]^{(Y \tdot)^ {s^0}} & &
	(Y \tdot)^{\Delta[1]}
}
\end{equation}
so it would be enough to prove that 
\begin{equation}
\label{eqnBK6}
{\bf R}{\lim}^\Delta (Y \tdot)^{\Delta[0]}
\xymatrix{
	 \ar[rr]_\sim^{{\bf R}{\lim}^\Delta (Y \tdot)^{s^0}} & &
}
{\bf R}{\lim}^\Delta (Y \tdot)^{\Delta[1]}
\end{equation}
is an equivalence.

To prove (\ref{eqnBK6}) we need two steps.

\bigskip

Step 1: Suppose we know (\ref{eqnBK6}) for constant complicial objects $Y \tdot$ = $cA$, where $A$ is a simplicial set.
Then we are going to prove it in the general case.

We add a constant vertical cosimplicial dimension in (\ref{eqnBK8}), and consider the map of bicosimplicial objects
\begin{center}
$\xymatrix{
	c(Y^{\Delta[0]}) \ar[rr]^{c(Y^{s^0})} & &
	c(Y^{\Delta[1]})
}$
\end{center}
where $cA$, $A \in Ob{\cat M}$ denotes the constant cosimplicial space equal to $A$.

We denote $\Delta$ = $\Delta_{ve}$ the vertical part, and $\Delta$ = $\Delta_{ho}$ the horizontal part of $\Delta \times \Delta$.

We apply ${\bf R}{\lim}^{\Delta_{ve} \times \Delta_{ho}}$ to the map above

\begin{equation}
\label{eqnBK7}
{\bf R}{\lim}^{\Delta_{ve} \times \Delta_{ho}} c(Y^{\Delta[0]})
\xymatrix{
	 \ar[rr] & &
}
{\bf R}{\lim}^{\Delta_{ve} \times \Delta_{ho}} c(Y^{\Delta[1]})
\end{equation}

Using the factorization
\begin{center}
${\bf R}\lim^{\Delta_{ve} \times \Delta_{ho}}$ $\simeq$ ${\bf R}\lim^{\Delta_{ve}} {\bf R}\lim^{\Delta_{ho}}$
\end{center}
that computes first ${\bf R}\lim^{\Delta_{ho}}$ in the horizontal direction, we get that (\ref{eqnBK7}) is exactly (\ref{eqnBK6}).

Using the factorization in the other order
\begin{center}
${\bf R}\lim^{\Delta_{ve} \times \Delta_{ho}}$ $\simeq$ ${\bf R}\lim^{\Delta_{ho}} {\bf R}\lim^{\Delta_{ve}}$
\end{center}
since we assume we know (\ref{eqnBK6}) for constant cosimplicial objects it follows that the map in (\ref{eqnBK7}) is a weak equivalence.
This proves Step 1.

\bigskip

Step 2: Proof of (\ref{eqnBK6}) when $Y \tdot$ is a constant cosimplicial object $Y \tdot$ = $cA$, where $A$ is a simplicial set.

If $A.$ is a simplicial set, we have to show that the map below is an equivalence
\begin{center}
${\bf R}{\lim}^{\Delta} (A.\!^{\Delta[0]})
\xymatrix{
	 \ar[rr]_\sim^{{\bf R}{\lim}^\Delta{A.\!^{s^0}}} & &
}
{\bf R}{\lim}^{\Delta} (A. \!^{\Delta[1]})$
\end{center}
We may assume that $A.$ is fibrant.

This map can be rewritten (by Lemma \ref{lemmaHCM4})
\begin{center}
$tot (A. \!^{\Delta[0]})  
\xymatrix{
	 \ar[r]^{tot (A.\!^{s^0})} &
}
tot (A. \!^{\Delta[1]})$
\end{center}
which by Lemma \ref{lemmaHCM2} is rewritten as the weak equivalence
\begin{center}
$hom (\Delta[0] \, , A.)
\xymatrix{
	 \ar[r]_\sim^{hom (s^0, A.)} &
}
hom (\Delta[1] \, , A.)$
\end{center}
\end{proof}

As a complement to the last two theorems, we have:
\begin{thm}
\label{thmHomot3}
If $f$ $\simeq$ $g$: $X. \lra Y.$ in ${\cat M}^{\Delta^{op}}$ then
\begin{center}
${\bf cotot}_n f$ = ${\bf cotot}_n g$ 
\end{center}
for any $n \ge 1$.
\end{thm}

Dually
\begin{thm}
\label{thmHomot4}
If $f$ $\simeq$ $g$ : $X \tdot \lra Y \tdot$ in ${\cat M}^\Delta$ then
\begin{center}
${\bf tot}^n f$ = ${\bf tot}^n g$ 
\end{center}
for any $n \ge 1$.
\end{thm}

Note that these results are not true for $n$ = $0$.

\begin{proof}
The proof of both of these Theorems is parrallel to the proof of the two theorems before, so we will only sketch it.

First, one shows that it is enough to prove Theorem \ref{thmHomot4} for the case ${\cat M}$ = $sSets$.

Assume ${\cat M}$ = $sSets$ let's sketch the proof Theorem \ref{thmHomot4}.
If $Y \tdot$ is a cosimplicial space, the proof reduces to showing that the map
\begin{equation}
\label{eqnBK10}
{\bf tot}^n (Y \tdot)^{\Delta[1]}
\xymatrix{
	 \ar[rr]_\sim^{{\bf tot}^n (Y \tdot)^{s^0}} & &
}
{\bf tot}^n (Y \tdot)^{\Delta[0]}
\end{equation}
is an equivalence.

Similarly to Step 1 in the proof before, this further reduces to proving (\ref{eqnBK10}) in the particular case when $Y \tdot$ is a constant cosimplicial object $Y \tdot$ = $cA$, where $A$ is a simplicial set.

If $A.$ is a simplicial set, we have to show that the map below is an equivalence
\begin{center}
${\bf tot}^n (A.\!^{\Delta[0]})
\xymatrix{
	 \ar[rr]_\sim^{{\bf tot}^n {A.\!^{s^0}}} & &
}
{\bf tot}^n {\lim} (A. \!^{\Delta[1]})$
\end{center}
We may assume that $A.$ is fibrant.

This map can be rewritten (by Lemma \ref{lemmaHCM4})
\begin{center}
$tot^n (A. \!^{\Delta[0]})  
\xymatrix{
	 \ar[r]^{tot^n (A.\!^{s^0})} &
}
tot^n (A. \!^{\Delta[1]})$
\end{center}
which by Lemma \ref{lemmaHCM3} is rewritten as 
\begin{center}
$hom (sk_n \Delta[0] \, , A.)
\xymatrix{
	 \ar[r]^{hom (s^0, A.)} &
}
hom (sk_n \Delta[1] \, , A.)$
\end{center}
This last map is an equivalence, because $sk_n \Delta[1] \ra sk_n \Delta[0]$ is an equivalence for $n \ge 1$.
\end{proof}

